Workflow Mini-Apps: Portable, Scalable, Tunable & Faithful Representations of Scientific Workflows

Workflows are critical for scientific discovery. However, the sophistication, heterogeneity, and scale of workflows make building, testing, and optimizing them increasingly challenging. Furthermore, their complexity and heterogeneity make performance reproducibility hard. In this paper, we propose workflow mini-apps as a tool to address the challenges in building and testing workflows while controlling the fidelity of representing realworld workflows. Workflow mini-apps are deployed and run on various HPC systems and architectures without workflow-specific constraints. We offer insight into their design and implementation, providing an analysis of their performance and reproducibility. Workflow mini-apps thus advance the science of workflows by providing simple, portable, and managed (fidelity) representations of otherwise complex and difficult-to-control real workflows.

==> motivation.tex <==
% !TeX root = main.tex


\ozgurnote{I will be rewriting motivation by focusing on where mini-apps can be useful and how.}



Developing a scientific workflow is
% even more
challenging since scientific workflows combine many sets of tasks with possibly distinct requirements, such as specific libraries, CPU (e.g., x86, PowerPC), and GPU (e.g., Nvidia, AMD)  architectures,
accelerators, and more. Complexity increases with communication and dependencies within and between those sets of tasks. With increased complexity and heterogeneity, testing a workflow becomes more complicated and time-consuming, hence costly. 
We propose workflow mini-apps to reduce the cost and complexity of developing and testing scientific workflows.


Workflow mini-apps provide several advantages for developing, testing, deploying, and optimizing scientific workflows. 

We created four main categories (performance reproducibility, portability, scalability, and testing the execution on new HPC platforms or new execution models) on how workflow mini-apps can benefit the scientific computing community. For this purpose, our workflow mini-apps balance the trade-off between simplicity, portability, and fidelity.

Performance reproducibility becomes challenging with increased heterogeneity and complexity of the workflows. To test it, one will need original data, the exact runtime environment, workflow execution/submission scripts, and all additional constraints. Even if all of them are available, it will also require running the original workflow multiple times, a costly endeavor. %ADD REference 
Workflow mini-apps solve this by reducing the makespan (a fixed and adjustable ratio of the original workflow's runtime) while providing performance fidelity (comparable internal performance, such as resource and I/O utilization of each task and application within the workflow). 



Portability is another issue for workflows. For example, the initial workflow we used (Inverse Problem from ExaLearn~\cite{wang2023parallel}) depends on GSAS-II library~\cite{toby2013gsas}, which can only run on a specific architecture. Workflow mini-apps allow for the exploration and evaluation of new architectures by removing constraints and dependencies to particular libraries, OSs, and CPU/GPU architectures while maintaining fidelity. Running workflow mini-apps on various platforms with different architectures
provides initial performance results so that scientists can decide if it is worth implementing their workflow using a different library that is supported by a specific platform.

Similar to portability, it is crucial to test whether scaling the workflow up is worth the cost. In some cases (e.g., where there is a lot of I/O or communication between tasks), scaling up may not benefit or even hurt the workflow performance. Scientists would run the original workflow with higher resources and check the results to test the performance, which would become costly. However, the workflow mini-app can provide performance metrics of scaled-up execution using a shorter time than the workflow itself.

One can also improve the performance of the workflow by changing the execution model.
Workflow mini-apps provide performance metrics such as makespan, and resource and I/O utilization to show the possible performance of the new execution model. Workflow mini-apps use pilot-based~\cite{turilli2018comprehensive} execution middleware RADICAL Ensemble Toolkit (EnTK)~\cite{entk2016bala} and RADICAL Pilot (RP)~\cite{merzky2021design} to enable  scalability of the heterogeneous workflows and also ease of implementing different execution models 


==> rebuttal_IPDPS.tex <==
% !TeX root = main.tex
\ozgurnote{Max 1000 word}


\subsection{General Complains}
Problem 1: Usability needs to be improved. Creating Mini-apps would require deep understanding of the workflow and learning tools like Darshan and RCT

Problem 2: There is lack of  Generality. 

\subsection{Reviewer 1's Feedback}
\begin{itemize}
    \item Need more detail on usability
    \item Need more explanation of Results
    \item Need more explanation how to use API to emulate workflows
    \item Explain more why not "Sleep"
    \item Not easy to build since needs deep understanding of workflow.
    \item Hard to implement
    \item Require learning tools such RCT and Darshan
    \item No automated profiling 
    \item Mini-apps are not mini only 2X smaller 
    \item Need 3-5 runs for fine tuning
    \item Need to show fine tuning in experiments. 
    \item It would be good to have a code sample with parameters for fine tuning
    \item section 5.5 needs more explanation such as what are the steps required to do this
    \item Section 5.3 needs more explanation of portability.  and it would be good to add missing DDMD portability figure. 
\end{itemize}

\subsection{Reviewer 2's Feedback}
\begin{itemize}
    \item Deep knowladge needed to create mini-apps
    \item Better presentation of results would be good
    \item Table 2 and 3 could make it clearer
    \item Maybe leave out the Serial CPU data for the Inverse Problem workflow
    \item How exactly is the makespan/IO ratio of original workflow vs. proxy workflow determined? Is this configurable when designing the workflow miniapp or at runtime? How does it affect accuracy?
    \item What exactly do the resource usage diagrams (e.g. Fig 4a-f) depict? I assume it denotes which CPU/GPU is active at a given time during execution?
    \item Is it possible to distinguish the individual tasks (e.g. by color)
\end{itemize}


\subsection{Reviewer 3's Feedback}
\begin{itemize}
    \item It is not generic enough
    \item Development time needs to shorten
    \item Require deep understanding of original workflow
    \item Not every aspect of the workflow is considered.
    \item how different parameters affect performance
    \item Any modification of original workflow might result redesigning mini-app
\end{itemize}

\subsection{Reviewer 4's Feedback}
\begin{itemize}
    \item lack of generality
    \item only eligible to use with RCT
    \item Portability would be better to show fidelity by also running the original task in the new system 
    \item No root cause analysis for performance variation.
    \item Better Formation on tables and figures
    \item Performance portability is not provided and explained
\end{itemize}

\subsection{Rebuttal text}

We want to thank the reviewers for their time and comments.  We understand that a few common comments are shared by all the reviewers: the need for more generality and a better explanation of usability. 
We recognized that Workflow mini-apps are not universal and require an understanding of the original workflow to develop. We will add a section to discuss what our tool focuses on (Our tool mainly focuses on reducing the cost of the testing and improving the workflow, and to do so, we need to provide high fidelity in terms of the selected performance metrics)  and how our tool can be used (e.g., Why we used RCT and Darshan and how can you change them, how one can use proposed API to build Emulated tasks easily.).  We will also work on our figures and table to make them easier to understand and add missing figures regarding DeepDriveMD portability and more. 

\paragraph{Answer reviewer 1's feedback:} (Why not Sleep) We extend the explanation we presented in 4.2. (No automated Profiling) We are working towards integrating profiling tools for our future work. 
(mini-apps are not mini) We choose to scale by 2X for DeepDriveMD and 4X for Inverse Problem due to their total run time and run time of each task; one can pick any other scale.  (Detail about fine-tuning) We will purchase extra pages to provide more details about each step with example codes. Also, we have an open-source GitHub directory where we share our entire code base.

\paragraph{Answer reviewer 2's feedback:} (how ratio decided) We used the total run time of each task and entire workflow to decide how much we want to shorten the run time, and we will explain that in more detail. Also, we are planning to use color codes for each task type in the figures.

\paragraph{Answer reviewer 3's feedback:} (long development time) Fine-tuning only needs to run mini-apps multiple times, which are not costly to run. (Not every aspect considered) we consider some of the most important aspects to provide performance representation with minimal complexity. Every additional aspect would increase the complexity of mini-apps.  (any modification to workflow results in re-designing mini-apps) this depends on the modification. Some may need only to change parameters, and others will require rewriting. For this, our API provides generic kernels for specific types of overheads, and users only need to replace the changed kernel.

\paragraph{Answer reviewer 4's feedback:} (better portability experiments needed) We will provide more experiments suggested by the reviewer to show the fidelity of the mini-apps based on portability. 

Again, we thank all the reviewer for their time, and we hope we were able to answer every concern from them.


\subsection{TODO:}
\begin{itemize}
    \item create a Google doc for what we need to do
    \item Convert the paper to IEEE format. 
    \item Rework the text
    \begin{itemize}
        \item Be more clear on purpuse of the workflow mini-apps
        \item Address the Generality
        \item Add a subsection for usability
        \item 
    \end{itemize}
    \item work on the figures. 
    \item 
\end{itemize}

% contribution / and need 
% What is the mini-app
% Provide the artifact  We need c
% Be more clear  and preemt the attach by attacking 
%     Maybe say it looks like this but it is that .. 
%     we need to be more clear and reduce the size. 
    

==> usagearea.tex <==
% !TeX root = main.tex
Workflow Mini-Apps are needed to address the challenges of building, testing, and deploying scientific workflows. For example, a need to build workflow mini-apps mentioned in the High Energy Physics Center for Computational Excellence (HEP-CCE) Status and Planning Report as part of the HEP-CCE 5-year plan~\cite{hepccereport2023indigo,hepccerwebpage}. This plan includes building various workflow mini-apps for HEP experiments such as ATLAS~\cite{aad2008atlas}, DUNE~\cite{abi2020volume}, and more. According to the HEP-CCE plan, workflow mini-apps will provide key performance metrics for future HPC facilities and help the experiment easily leverage new architectures.   
%
To show the possible advantages of Workflow mini-apps, we created five main categories: performance reproducibility, portability, exploring the performance on new HPC platforms, scalability, and testing the performance of new execution models. 

Workflow mini-apps address the challenges of performance reproducibility mentioned in \S~\ref{sec:intro} by reducing the makespan (a fixed and adjustable ratio of the original workflow's runtime) while providing performance fidelity (comparable internal performance, such as resource and I/O utilization of each task and application within the workflow). 

Workflow mini-apps allow for exploring and evaluating new architectures by removing constraints and dependencies to particular libraries, OSs, and CPU/GPU architectures while maintaining fidelity.
For example, the original Inverse Problem workflow from ExaLearn~\cite{wang2023parallel} depends on the GSAS-II library~\cite{toby2013gsas}, which can only run on a specific architecture. 
Running workflow mini-apps on various platforms with different architectures provides initial performance results so that scientists can decide if it is worth implementing their workflow using a different library that is supported by a specific platform.

It is also crucial to test the scaling of the workflows. In some cases (e.g., where there is a lot of I/O or communication between tasks), scaling up may not benefit or even hurt the workflow performance. Workflow mini-app can provide performance metrics of scaled-up execution using a shorter time than the workflow itself and reducing the cost.

One can also improve the performance of the workflow by changing the execution model.
Workflow mini-apps provide performance metrics such as makespan and resource and I/O utilization to show the possible performance of the new execution model.  We used the DeepDriveMD workflow mini-app to test an asynchronous execution model. 
